On the Surprising Robustness of Sequential Convex Optimization for Contact-Implicit Motion Planning

Contact-implicit motion planning-embedding contact sequencing as implicit complementarity constraints-holds the promise of leveraging continuous optimization to discover new contact patterns online. Nevertheless, the resulting optimization, being an instance of Mathematical Programming with Complementary Constraints, fails the classical constraint qualifications that are crucial for the convergence of popular numerical solvers. We present robust contact-implicit motion planning with sequential convex programming (CRISP), a solver that departs from the usual primal-dual algorithmic framework but instead only focuses on the primal problem. CRISP solves a convex quadratic program with an adaptive trust region radius at each iteration, and its convergence is evaluated by a merit function using weighted penalty. We (i) provide sufficient conditions on CRISP's convergence to first-order stationary points of the merit function; (ii) release a high-performance C++ implementation of CRISP with a generic nonlinear programming interface; and (iii) demonstrate CRISP's surprising robustness in solving contact-implicit planning with naive initialization. In fact, CRISP solves several contact-implicit problems with all-zero initialization.

==> sections/app-toy-example.tex <==
\section{Another CQs fail Example}
\label{app:toy-cq-fail}
In this section, we consider the following 2D minimization problem:
\begin{align}
    \label{eq:case:problem}
    \min_{x_1,x_2} & \displaystyle \,\,\,x_1 \notag\\
    \subject &\,\, x^3_1-x_2 \geq 0,\\
    & \,\, x^3_1+x_2 \geq 0.\notag
\end{align}
The objective level set and the feasible region are visualized in \prettyref{fig:prob_illustration}. From the figure, we shall easily observe that the optimal solution lies at $x^*=(0,0)$. Let the objective and the constraints in (\ref{eq:case:problem}) be $f(x)$, $c_1(x)$ and $c_2(x)$ respectively, we have:

\begin{equation}
\nabla f\left(x\right)=\left[\begin{array}{l}
1 \\
0
\end{array}\right], \quad \nabla c_1\left(x\right)=\left[\begin{array}{c}
3x_1^2\\
-1
\end{array}\right], \quad \nabla c_2\left(x\right)=\left[\begin{array}{c}
3x_1^2 \\
1
\end{array}\right].
\end{equation}
At the optimal point $x^*$, the gradients of the two constraints are linearly dependent ($\nabla c_1(x^*)=[0,-1]^{\top}$ and $\nabla c_2(x^*)=[0,1]^{\top}$), causing the Linear Independence Constraint Qualification (LICQ) to fail. LICQ is typically required for the KKT system to provide necessary first-order optimality conditions~\cite{nocedal1999springer-numerical-optimization}. While alternative constraint qualifications exist that can yield analogous optimality conditions, a direct examination of the Lagrangian gradient $\nabla_x \mathcal{L}$ at the optimal point $x^*$ reveals the failure of the KKT conditions. Specifically, there exist no Lagrange multipliers $\lambda_1$ and $\lambda_2$ that satisfy:
\begin{equation}
    \nabla f(x^*) - \lambda_1 \nabla c_1(x^*) -\lambda_2 \nabla c_2(x^*) = \left[\begin{array}{c}
         1 \\
         \lambda_1 -\lambda_2 
    \end{array}\right] = \mathbf{0}.
\end{equation}
In this section, we conduct a comprehensive analysis of our proposed algorithm's performance on this typical problem, encompassing both theoretical investigation and numerical experiments.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.2\textwidth, trim={5cm 9cm 5cm 9cm}, clip]{figures/toy_appendix.pdf}
    \caption{Visualization of the objective level sets (red lines) and the feasible region (shaded area).}
    \label{fig:prob_illustration}
\end{figure}
\paragraph{Convergency Analysis} Starting from an initial point $\boldsymbol{x}_0$, we implement Algorithm \ref{alg:sl1qp:modified} on the problem (\ref{eq:case:problem}) recursively to obtain a sequence of $\boldsymbol{x}$. Suppose we are now at $\boldsymbol{x}_k$, a trial step $\hat{\boldsymbol{p}}_k = [\hat{p}_{k,1},\hat{p}_{k,2}]$ at each iteration $k$ by solving:
\begin{align}\label{eq:case:subproblem_k}
\min_{\hat{\boldsymbol{p}}} \, & \quad x_1 + \hat{p}_1 + \mu[x_1^3-x_2+3x_1^2\hat{p}_1-\hat{p}_2]^- + \mu[x_1^3+x_2+3x_1^2\hat{p}_1+\hat{p}_2]^-\\
\subject & \quad \norm{\hat{\boldsymbol{p}}_k}_\infty \leq \Delta_k.\notag
\end{align}
For simplicity, we abbreviate the explicit dependence of certain variables on the iteration number $k$. Given that~\eqref{eq:sl1qp:sl1qp-subproblem} is merely a smooth reformulation of~\eqref{eq:case:subproblem_k} with an identical minimizer, we focus our analysis on the non-smooth version, which offers greater analytical tractability. The optimal trial step, which minimizes the objective function while adhering to the trust-region constraint, is contingent upon three key factors: the chosen penalty parameter $\mu$, the current position $(x_1, x_2)$, and the trust-region radius determined in the outer loop.




Denote the two penalty terms in~\eqref{eq:case:subproblem_k} as $m_{\mu}$, we rearrange it as:
\begin{equation}
    m_{\mu} = \mu[x_1^2(x_1+3\hat{p}_1)-(x_2+\hat{p}_2)]^- + \mu[x_1^2(x_1+3\hat{p}_1)+(x_2+\hat{p}_2)]^-.
\end{equation}
Given that the terms beyond $m_{\mu}$ are independent of $\hat{p}_2$, we first focus our analysis on determining the optimal value of $\hat{p}_2$ that minimizes $m_{\mu}$. From the symmetric characteristic of the two terms, we can infer that: 
\begin{align}
x_1 + 3p_1 \leq 0 &\Rightarrow \textbf{Take}\,\begin{array}{c}
     |x_2+\hat{p}_2| \leq -x_1^2(x_1 + 3\hat{p}_1)  \\
     \&\&\,|\hat{p}_2\leq\Delta_k|
\end{array} \Rightarrow \min m_{\mu}=2\mu(-x_1^2(x_1+3\hat{p}_1)), \label{eq:case:mu_1}\\
x_1 + 3p_1 > 0 &\Rightarrow \textbf{Take}\,\begin{array}{c}
     |x_2+\hat{p}_2| \leq x_1^2(x_1 + 3\hat{p}_1)  \label{eq:case:mu_2}\\
     \&\&\,|\hat{p}_2\leq\Delta_k|
\end{array} \Rightarrow \min m_{\mu}=0.
\end{align}

Note that if the set inside ``\textbf{Take}'' is $\emptyset$, then $p_2 = -\mathrm{sign}(x_2)\Delta_k$. This implies that the absolute value of $x_2$ is monotonically decreasing. Consequently, after a finite number of iteration, the set will become non-empty. 

Combining the cases in~\eqref{eq:case:mu_1} and~\eqref{eq:case:mu_2}, we rewrite the objective in~\eqref{eq:case:subproblem_k} by taking appropriate value on $\hat{p}_2$:
\begin{equation}
\label{eq:case:subproblem_k_min}
\min_{\hat{p}_1} \,  \quad x_1 + \hat{p}_1 - \min\{0,2\mu(x_1^2(x_1+3\hat{p}_1))\},
\end{equation}
where we can absorb all terms in the $\min$ operator and disregard the constant $x_1$ to further simplify it to a \textit{min-max} form:
\begin{equation}
\label{eq:case:subproblem_k_simplify1}
\min_{\hat{p}_1} \max\{\hat{p}_1,\hat{p}_1-2\mu(x_1^2(x_1+3\hat{p}_1))\},\,|\hat{p}_1|\leq \Delta_k.
\end{equation}
\begin{center}
$\downarrow$
\end{center}
\begin{equation}
\label{eq:case:subproblem_k_simplify2}
\min_{\hat{p}_1} \max\{\hat{p}_1,(1-6\mu x_1^2)\hat{p}_1-2\mu x_1^3\},\,|\hat{p}_1|\leq \Delta_k.
\end{equation}
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.30\textwidth}
  \centering
%%%    \begin{adjustbox}{width=\linewidth} % rescale box
    \begin{tikzpicture}
% Axes
    \draw[->] (-2,0) -- (2,0) node[right] {$p_1$}; % x-axis
    \draw[->] (0,-3) -- (0,3) node[above] {$y$}; % y-axis

    % Adjustable x1 value
    \def\xone{0.5} % Set x1 value (you can adjust this)

    % Vertical line for x = x1
    \draw[thick, dashed] (1,-3) -- (1,3); % x1 vertical line
    \node[below right] at (1,0) {$\Delta_k$};

    % Vertical line for x = x1
    \draw[thick, dashed] (-1,-3) -- (-1,3); % x1 vertical line
    \node[below right] at (-2.2,0) {$-\Delta_k$};

    % Line 1
    \draw[thick, domain=-1.5:1.5, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 2*(\xone)^3}); % 
    \draw[line width=3pt, domain=-1:-\xone/3, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 2*(\xone)^3});
    \node[above] at (-1.5,0.5) {$(1 - 6\mu x_1^2)p_1 - 2\mu x_1^3$};

    % Line 2
    \draw[thick, domain=-1.5:1.5, samples=100] 
        plot (\x, \x); 
    \draw[line width=3pt, domain=-\xone/3:1, samples=100] 
        plot (\x, \x);
    \node[above] at (1.5,0.5) {$p_1$};

     % Red point at (1, 1)
    \filldraw[red] (-\xone/3,-\xone/3) circle (2pt); % Draws a red filled circle at (1, 1)

    % Label for the red point
    \node[above right] at (-\xone/3-0.5,-\xone/3-1) {optimal };

    \end{tikzpicture}
%%%  \end{adjustbox}       %
\end{subfigure}%
   \hspace{0.02\textwidth}
  \begin{subfigure}[b]{0.30\textwidth}
  \centering
  \begin{tikzpicture}
% Axes
    \draw[->] (-2,0) -- (2,0) node[right] {$p_1$}; % x-axis
    \draw[->] (0,-3) -- (0,3) node[above] {$y$}; % y-axis

    % Adjustable x1 value
    \def\xone{0.6} % Set x1 value (you can adjust this)

    % Vertical line for x = x1
    \draw[thick, dashed] (1,-3) -- (1,3); % x1 vertical line
    \node[below right] at (1,0) {$\Delta_k$};

    % Vertical line for x = x1
    \draw[thick, dashed] (-1,-3) -- (-1,3); % x1 vertical line
    \node[below right] at (-2.2,0) {$-\Delta_k$};

    % Line 1
    \draw[thick, domain=-2:0.2, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 12*(\xone)^3}); % 
    \node[above] at (-0.8,-2.5) {$(1 - 6\mu x_1^2)p_1 - 2\mu x_1^3$};

    % Line 2
    \draw[thick, domain=-1.5:1.5, samples=100] 
        plot (\x, \x); 
    \draw[line width=3pt, domain=-1:1, samples=100] 
        plot (\x, \x);
    \node[above] at (1.5,0.5) {$p_1$};

     % Red point at (1, 1)
    \filldraw[red] (-1,-1) circle (2pt); % Draws a red filled circle at (1, 1)

    % Label for the red point
    \node[above right] at (-1,-1.5) {optimal };

    \end{tikzpicture}
%%%  \end{adjustbox}       %
\end{subfigure}%
\hspace{-0.01\textwidth}
\begin{subfigure}[b]{0.30\textwidth}
\centering
  \begin{tikzpicture}
% Axes
    \draw[->] (-2,0) -- (2,0) node[right] {$p_1$}; % x-axis
    \draw[->] (0,-3) -- (0,3) node[above] {$y$}; % y-axis

    % Adjustable x1 value
    \def\xone{-0.6} % Set x1 value (you can adjust this)

    % Vertical line for x = x1
    \draw[thick, dashed] (1,-3) -- (1,3); % x1 vertical line
    \node[below right] at (1,0) {$\Delta_k$};

    % Vertical line for x = x1
    \draw[thick, dashed] (-1,-3) -- (-1,3); % x1 vertical line
    \node[below right] at (-2.2,0) {$-\Delta_k$};

    % Line 1
    \draw[thick, domain=-0.2:2, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 12*(\xone)^3}); % 
      \draw[line width=3pt, domain=-0.2:1, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 12*(\xone)^3});  
    \node[above] at (-0.8,0.5) {$(1 - 6\mu x_1^2)p_1 - 2\mu x_1^3$};

    % Line 2
    \draw[thick, domain=-1.5:1.5, samples=100] 
        plot (\x, \x); 

    \node[above] at (1.5,0.5) {$p_1$};

     % Red point at (1, 1)
    \filldraw[red] (1,1.5) circle (2pt); % Draws a red filled circle at (1, 1)

    % Label for the red point
    \node[above right] at (1,1.5) {optimal };

    \end{tikzpicture}
%%%  \end{adjustbox}       %
\end{subfigure}%
\caption{Visualization of cases where $1-6\mu x_1^2 \leq 0$. The graph illustrates three distinct scenarios, each corresponding to different values of $x_1$, showcasing the various intersections of the two linear functions. The bold segments represent the composite \textit{max} function, while the \textit{min} points are denoted by red dots. The intersection is $\hat{p}_1 = -x_1/3$.}
\label{fig:case-visualization01}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.30\textwidth}
  \centering
%%%    \begin{adjustbox}{width=\linewidth} % rescale box
    \begin{tikzpicture}
% Axes
    \draw[->] (-2,0) -- (2,0) node[right] {$p_1$}; % x-axis
    \draw[->] (0,-3) -- (0,3) node[above] {$y$}; % y-axis

    % Adjustable x1 value
    \def\xone{0.3} % Set x1 value (you can adjust this)

    % Vertical line for x = x1
    \draw[thick, dashed] (1,-3) -- (1,3); % x1 vertical line
    \node[below right] at (1,0) {$\Delta$};

    % Vertical line for x = x1
    \draw[thick, dashed] (-1,-3) -- (-1,3); % x1 vertical line
    \node[below right] at (-2.2,0) {$-\Delta$};

    % Line 1
    \draw[thick, domain=-1.5:1.5, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 2*(\xone)^3}); % 
    \draw[line width=3pt, domain=-1:-\xone/3, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 2*(\xone)^3});
    \node[above] at (-1.5,0.5) {$(1 - 6\mu x_1^2)p_1 - 2\mu x_1^3$};

    % Line 2
    \draw[thick, domain=-1.5:1.5, samples=100] 
        plot (\x, \x); 
    \draw[line width=3pt, domain=-\xone/3:1, samples=100] 
        plot (\x, \x);
    \node[above] at (1.5,0.5) {$p_1$};

     % Red point at (1, 1)
    \filldraw[red] (-1,-1 + 6*\xone^2 - 2*\xone^3) circle (2pt); % Draws a red filled circle at (1, 1)

    % Label for the red point
    \node[above right] at (-1.5,-1 + 6*\xone^2 - 2*\xone^3-1) {optimal };

    \end{tikzpicture}
%%%  \end{adjustbox}       %
\end{subfigure}%
   \hspace{0.02\textwidth}
  \begin{subfigure}[b]{0.30\textwidth}
  \centering
  \begin{tikzpicture}
% Axes
    \draw[->] (-2,0) -- (2,0) node[right] {$p_1$}; % x-axis
    \draw[->] (0,-3) -- (0,3) node[above] {$y$}; % y-axis

    % Adjustable x1 value
    \def\xone{0.25} % Set x1 value (you can adjust this)

    % Vertical line for x = x1
    \draw[thick, dashed] (1,-3) -- (1,3); % x1 vertical line
    \node[below right] at (1,0) {$\Delta$};

    % Vertical line for x = x1
    \draw[thick, dashed] (-1,-3) -- (-1,3); % x1 vertical line
    \node[below right] at (-2.2,0) {$-\Delta$};

    % Line 1
    \draw[thick, domain=-2:1.5, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 36*(\xone)^3}); % 
    \node[above] at (-0.8,-2.5) {$(1 - 6\mu x_1^2)p_1 - 2\mu x_1^3$};

    % Line 2
    \draw[thick, domain=-2:1.5, samples=100] 
        plot (\x, \x); 
    \draw[line width=3pt, domain=-1:1, samples=100] 
        plot (\x, \x);
    \node[above] at (1.5,0.5) {$p_1$};

     % Red point at (1, 1)
    \filldraw[red] (-1,-1) circle (2pt); % Draws a red filled circle at (1, 1)

    % Label for the red point
    \node[above right] at (-1,-1) {optimal };

    \end{tikzpicture}
%%%  \end{adjustbox}       %
\end{subfigure}%
\hspace{-0.01\textwidth}
\begin{subfigure}[b]{0.30\textwidth}
\centering
  \begin{tikzpicture}
% Axes
    \draw[->] (-2,0) -- (2,0) node[right] {$p_1$}; % x-axis
    \draw[->] (0,-3) -- (0,3) node[above] {$y$}; % y-axis

    % Adjustable x1 value
    \def\xone{-0.25} % Set x1 value (you can adjust this)

    % Vertical line for x = x1
    \draw[thick, dashed] (1,-3) -- (1,3); % x1 vertical line
    \node[below right] at (1,0) {$\Delta$};

    % Vertical line for x = x1
    \draw[thick, dashed] (-1,-3) -- (-1,3); % x1 vertical line
    \node[below right] at (-2.2,0) {$-\Delta$};

    % Line 1
    \draw[thick, domain=-1.5:2, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 36*(\xone)^3}); % 
      \draw[line width=3pt, domain=-1:1, samples=100] 
        plot (\x, {(1 - 6*(\xone)^2)*\x - 36*(\xone)^3});  
    \node[above] at (-0.8,1) {$(1 - 6\mu x_1^2)p_1 - 2\mu x_1^3$};

    % Line 2
    \draw[thick, domain=-1.5:2, samples=100] 
        plot (\x, \x); 

    \node[above] at (1.5,0.5) {$p_1$};

     % Red point at (1, 1)
    \filldraw[red] (-1,-0.1) circle (2pt); % Draws a red filled circle at (1, 1)

    % Label for the red point
    \node[above right] at (-1,0) {optimal };

    \end{tikzpicture}
%%%  \end{adjustbox}       %
\end{subfigure}%
\caption{Visualization of cases where $1-6\mu x_1^2 > 0$. In all three scenarios depicted, the optimal solution converges to the same \textit{min-max} point at $\hat{p}_1=-\Delta$, regardless of the specific intersection patterns of the linear functions.}
\label{fig:case-visualization02}
\end{figure}
We then analyze different cases distinguished by the sign of $1-6\mu x_1^2$. For clarity, these scenarios are illustrated in~\prettyref{fig:case-visualization01}, which provides an intuitive understanding of the process. The figure demonstrates how we first identify the \textit{max} segment of these two lines and then extract the \textit{min} point of the resulting composite line, thereby solving the constrained \textit{min-max} problem. Thus, we conclude that:
\begin{align}
|x_1| > 1/\sqrt{6\mu} &\Rightarrow \hat{p}_1  = \mathrm{clip}(\frac{-x_1}{3},\Delta_k) \\
-1/\sqrt{6\mu}\leq x_1 \leq 1/\sqrt{6\mu} &\Rightarrow \hat{p}_1  = -\Delta_k,
\end{align}
which indicates that $\hat{p}_1$ will always take a step towards $x_1=-1/\sqrt{6\mu}$, either with length $|x_1/3|$ or the trust region radius $|\Delta_k|$. The \textbf{clip} function is defined by $\mathrm{clip}(a,b) = \max\{\min\{a,b\},-b\}$. Consequently, $x_2$ would converge to zero by taking the value consistent in Equation~\eqref{eq:case:mu_1} and~\eqref{eq:case:mu_2}. We thus conclude that the proposed algorithm exhibits dynamic convergence towards a final stable point, $(-1/\sqrt{6\mu},0)$.

The radius of the trust region is dynamically adjusted based on the magnitude of decrease in the merit function induced by the trial step. Through a similar deduction on the merit function, with an appropriately chosen $x_2$, we obtain:
\begin{equation}
    \phi_1 = x_1 + \mu[x_1^3-x_2]^-+\mu[x_1^3+x_2]^- = 
    \begin{cases}
        x_1 - 2\mu x_1^3,  & \text{for } x_1 < 0 \\
        x_1, & \text{for } x_1 \geq 0
    \end{cases}
\end{equation}
The stationary point of $\phi_1$ is obtained at $x_1 = -1/\sqrt{6\mu}$ and $|x_2|\leq|x_1^3|$. In practice, we employ a large value for $\mu$, resulting in $x_2$ being a negligibly small quantity, approaching zero due to the cubic relationship. This stationary point aligns with the stable point of our algorithm.

==> sections/experiments.tex <==
%!TEX root = ../main.tex

\section{Experiments}
\label{sec:exp}


\subsection{UW Rome Dataset}

\begin{itemize}
    \item No images
    
    \item Use original paper data (Bundle adjustment in the large) as GT
    
    \item Report
    \begin{enumerate}
        \item Baseline: \red{Ceres and GTSAM} (at least one of them)
        \item Accuracy of all methods (compared with GT, or we define new GT and show our GT is better, qualitatively)
        \item Suboptimality (\& min eig, cite Luca's early paper)
        \item Solver time (form $Q$ matrix time in Python + \nameshort solver time in GPU)
    \end{enumerate}

    \item Goal: the new formulation is better 
    \begin{enumerate}
        \item Faster than Ceres, GTSAM 
        \item Global, no initialization, compared with Ceres and GTSAM
    \end{enumerate}

    
    \item Appendix (more scientific)
    \begin{enumerate}
        \item When does the relaxation break? (1: depth is too noisy (add varying levels of depth noise) 2: outliers: random edges in the view graph)
    \end{enumerate}
\end{itemize}


\subsection{Replica Dataset}

\begin{itemize}
    \item With images
    \item GT camera pose
    \item Use GT depth
    \item Report
    \begin{enumerate}
        \item Baseline: COLMAP, GLOMAP
        \item Accuracy with respect to GT
        \item Suboptimality
        \item Solver time
    \end{enumerate}
    \item Goal:
    \begin{enumerate}
        \item Faster than COLMAP, GLOMAP
        \item Almost same accuray when using GT Depth 
        \item Potentially, when using monocular depth prediction, do \nameshort + Ceres/GTSAM
    \end{enumerate}
\end{itemize}

\subsection{Mip-Nerf + Zip-Nerf}

\nameshort, \nameshort + Ceres

Qualitative comparison with COLMAP

Novel view synthesis with all results

Appendix:
\begin{enumerate}
    \item What is the best monocular depth prediction model for \nameshort: DepthAnything, UniDepth, DepthPro
\end{enumerate}

\subsection{(Optional) ETH3D}

Has GT camera poses




\subsection{IMC}

\nameshort, \nameshort + Ceres

Qualitative comparison with COLMAP

\subsection{TUM}

\nameshort, \nameshort + Ceres

Qualitative comparison with COLMAP




==> sections/note.tex <==
%!TEX root = ../main.tex

\section{Note for discussion}
\label{sec:note}

\subsection{Jan 4}

\begin{itemize}
    \item Components
    \begin{enumerate}
        \item \teaser++: 3D-3D registration
        \item re\ransac: 2D-3D registration
        \item \glomap two-view filter: 3D-3D registration
    \end{enumerate}
    Finally we choose 
    \begin{enumerate}
        \item \nameshort purely as a baseline, denote by \nameshort
        \item \nameshort running for two times, denote by \xmdouble
        \item \xmdouble + re\ransac + \teaser++ as one pipline, denote by \xmdouble-T
        \item \xmdouble + \glomap two-view filter as another pipeline, denote by \xmdouble-F
    \end{enumerate}
    These three are all filters. These filter method now have the following thing we have not figured out:
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{red}{How to tune the hyper-parameters?}
        \item \textcolor{red}{It may cause the number of images decrease.}
        \item \textcolor{red}{It may make the view-graph sparse.}
    \end{enumerate}
    \item Neural rendering:
    Plan to use \colmap, seems glomap is not that stable.
    \item Breakdown plot
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{green}{Add solver time}
        \item \textcolor{green}{Remove \teaser + \ransac}
    \end{enumerate}
    \item Visualization
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{red}{Add circle rotation Visualization}
    \end{enumerate}
    \item Replica main table
    \begin{enumerate}[label={\checkmark}]
        \item \textcolor{green}{Change to median}
        \item \textcolor{green}{separate solve and propress time for glomap.}
    \end{enumerate}
    \item Suboptimality
    The math of suboptimility is here:
    For the problem with regularity term, the primal problem is:
    \begin{align}
    \min ~~&\langle C, X \rangle + Q(X)\\
    s.t. ~~&X \succ 0\\
    & \langle A_i, X \rangle = b_i, ~~\forall i
    \end{align}
    $Q(X)$ is a quadratic term defined by $Q(X) = \lambda \sum_i (X_{ii}-1)^2$. This is still a convex problem and the lagrangian is:
    \begin{align}
    L(X, y, Z) =& \langle C, X \rangle + Q(X) - \\&\sum_i y_i (\langle A_i, X \rangle - b_i) - \langle Z, X \rangle \\
    =& \langle C - \sum_i y_i A_i - Z, X \rangle + Q(X) + \sum_i y_i b_i
    \end{align}
    The KKT condition is:
    \begin{align}
    Z =& C + \nabla Q(X) - \sum_i y_i A_i \succ 0 \\
    \langle A_i, X \rangle =& b_i, ~~\forall i \\
    X \succ & 0 \\
    \langle Z, X \rangle = & 0
    \end{align}
    \red{For $Q(X) = 0$ I know to get $\inf L(X, y, Z)$  finite we need $C - \sum_i y_i A_i = Z \succ 0$. }
    Note $L$ is linear in the off-diagnol elements of $X$, and quadratic in the diagnol elements of $X$. To get the minimum finite, we need $(\nabla L)_{ij} = 0,~i\neq j$. For the diagnol elements, we need $(\nabla L)_{ij} = 0$ to get the minimal point. So together we will need $\nabla L = 0$, i.e.
    \begin{align}
    C - \sum_i y_i A_i - Z = -\nabla Q(X)
    \end{align}
    From diagnol we know $X_{ii} = -\frac{(C - \sum_i y_i A_i - Z)_{ii}}{2\lambda} + 1$. So we plug in $X$ then we get the dual problem:
    \begin{align}
    \max ~~&\sum_i b_i y_i - \frac{\sum_j (C - \sum_i y_i A_i - Z)_{jj}^2}{4\lambda} 
    \\ & + \sum_j (C - \sum_i y_i A_i - Z)_{jj} \\
    s.t. ~~&Z \succ 0\\
         ~~&(C - \sum_i y_i A_i - Z)_{ij} = 0, ~~i\neq j    
    \end{align}
    To derive the sub-optimality gap, we assume primal is feasible, then for all feasible $X$ we have:
    \begin{align}
    \langle C, X \rangle + Q(X) &\geq \langle C - \sum_i y_i A_i + \nabla Q(x) , X \rangle \\
    &+ \underbrace{\sum_i y_i b_i + Q(X) - \langle \nabla Q(X), X \rangle}_{\text{dual value}}\\
    &= \langle Z, X \rangle + p_{\text{dual}}\\
    &\geq \text{max}(0,\lambda_{\text{min}}(Z)) \text{tr}(X) + p_{\text{dual}}
    \end{align}
    then we define the sub-optimality gap as:
    \begin{align}
    p_{\text{primal}} - p_{\text{dual}} - \text{max}(0,\lambda_{\text{min}}(Z)) \text{tr}(X)
    \end{align}
\end{itemize}

\subsection{Jan 10}
\begin{itemize}
    \item Undistort images -- if it is radial camera, need to do undistortion
\end{itemize}


==> tables/conversion_speed.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        & \yalmip (Matlab) & \sostools (Matlab) & \tssos (Julia) & Ours (Matlab) \\
        \hline
        $N = 4$ & $8.18$s & $3.39$s & $2.40$s & $\bm{0.09}$\textbf{s} \\
        \hline 
        $N = 30$ & $68.89$s & $>30$min & $2.51$s & $\bm{0.32}$\textbf{s}  \\
        \hline
    \end{tabular}
    \vspace{1mm}
    \caption{POP-SDP conversion time of $4$ conversion packages in the inverted pendulum problem. When $N = 30$, \sostools takes more than $30$ miniutes and takes more than $300$GB memory.
    \label{tab:exp:gen:conversion-speed}}
\end{table}

==> tables/hyper_params.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \label{tab:exp:gen:hyper-params}
    \centering
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & $d_x$ & $d_u$ & $\text{deg}_{\max}$ & $N$ & $\text{size}(M)$ & $\#M$ & $\text{size}(L)$ & $\#L$ & $m_{\text{SDP}}$ & $\log_{10}\xi$ \\
        \hline 
        Inverted Pendulum & $4$ & $1$ & $2$ & $30$ & $55$ & $30$ & $10$ & $60$ & $47351$ & $\bm{-2.58}$ ($\bm{-2.93}$) \\
        \hline 
        Cart-Pole & $5$ & $1$ & $2$ & $30$ & $105$ & $30$ & $14$ & $273$ & $168961$ & $\bm{-2.89}$ ($\bm{-2.98}$) \\
        \hline 
        Car Back-in & $4 (+3)$ & $4$ & $3$ & $30$  & $190$ & $30$ & $19$ & $659$ & $509141$ & $\bm{-1.87}$ ($\bm{-1.99}$) \\
        \hline 
        Vehicle Landing & $8$ & $2$ & $2$ & $50$ & $190$ & $50$ & $19$ & $499$ & $946326$ & $\bm{-2.47}$ ($\bm{-2.42}$) \\
        \hline 
        Flying Robot & $8$ & $4$ & $2$ & $60$ & $231$ & $60$ & $21$ & $659$ & $1595001$ & $\bm{-2.57}$ ($\bm{-2.49}$) \\
        \hline 
    \end{tabular}
    }

    \caption{Hyper-parameters and suboptimality gaps in five numerical experiments. Means (medians) are reported for suboptimality gaps from \cuadmm. In the car back-in case, $(+3)$ denotes the $(A,B,C)$ parameters in the separation line.}
\end{table}

==> tables/onlyone.tex <==
%!TEX root = ../main.tex

\begin{table*}[htbp]
    \centering
    \resizebox{\textwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{} & \multirow{2}{*}{$d_x$} &\multirow{2}{*}{$d_u$} & \multirow{2}{*}{$\text{size}(M)$} & \multirow{2}{*}{$\#M$} & \multirow{2}{*}{$\text{size}(L)$} & \multirow{2}{*}{$m$} & \multirow{2}{*}{$\log_{10}\xi$} & \multicolumn{4}{c|}{Total Time} \\
        \cline{9-12}
        & & & & & & & & \mosek & \cdcs & \sdpnal & \cuadmm \\
        \hline 
        \multirow{2}{*}{Pendulum} & \multirow{2}{*}{$4$} & \multirow{2}{*}{$1$} & \multirow{2}{*}{$55$} & \multirow{2}{*}{$30$} & \multirow{2}{*}{$10$} & \multirow{2}{*}{$47351$} & $\bm{-2.58}$ ($\bm{-2.93}$) &  \multirow{2}{*}{$9.5$s} & \multirow{2}{*}{$110.3$s} & cold: $264.4$s & cold: $31.2$s ($14.6$s) \\
        \cline{8-8} \cline{11-12}
        & & & & & & & $\bm{-2.71}$ ($\bm{-2.97}$) & & & warm: $2.95$s & warm: \textbf{$\bm{0.66}$s} (\textbf{$\bm{0.62}$s}) \\
        \hline 
        Cart-Pole & $5$ & $1$ & $105$ & $30$ & $14$ & $168961$ & $\bm{-2.89}$ ($\bm{-2.98}$) & \textbf{$\bm{112.0}$s} & $1471$s & $3671$s & $183.0$s ($173.1$s) \\
        \hline 
        Car Back-in & $7$ & $4$ & $190$ & $30$ & $19$ & $509141$ & $\bm{-1.87}$ ($\bm{-1.99}$) & $>5$h & $6123$s & $>5$h & \textbf{$\bm{431.5}$s} (\textbf{$\bm{536.8}$s})  \\
        \hline 
        Vehicle Landing & $8$ & $2$ & $190$ & $50$ & $19$ & $946326$ & $\bm{-2.47}$ ($\bm{-2.42}$)  & $>5$h & $2.9$h & $>5$h &  \textbf{$\bm{919.2}$s} (\textbf{$\bm{1165}$s}) \\
        \hline 
        Flying Robot & $8$ & $4$ & $231$ & $60$ & $21$ & $1595001$ & $\bm{-2.57}$ ($\bm{-2.49}$) & $**$ & $>5$h & $>5$h & \textbf{$\bm{1648}$s} (\textbf{$\bm{2027}$s}) \\
        \hline 
    \end{tabular}
    }
    \vspace{0.5mm}
    \caption{Summary of numerical experiments. $(\text{size}(M), \#M)$: (dimension, number) of the moment matrices; $\text{size}(L)$: dimension of the localizing matrix. $m$: number of equality constraints in SDP.  Means (medians) are reported for $\log_{10}$ of suboptimality gaps $\xi$, and total running time of \cuadmm. 
    % The pendulum row lists total time with (upper) and without (lower) warmstarts. In the flying robot row,
    ``$**$'' indicates \mosek runs out of 1TB memory.
    \label{tab:exp:gen:onlyone}}
    \vspace{-10mm}
\end{table*}


==> tables/timing.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \label{tab:exp:gen:timing}
    \centering
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{} & \multicolumn{4}{c|}{Per-Iteration Cost} & \multicolumn{4}{c|}{Total Time} \\
        \cline{2-9}
        & \mosek & \cdcs & \sdpnal & \cuadmm & \mosek & \cdcs & \sdpnal & \cuadmm \\
        \hline 
        \multirow{2}{*}{Inverted Pendulum} & \multirow{2}{*}{$0.5$s} & \multirow{2}{*}{$11.1$ms} & \multirow{2}{*}{$59.1$ms} & \multirow{2}{*}{\textbf{$\bm{8.9}$ms}} & \multirow{2}{*}{$9.5$s} & \multirow{2}{*}{$110.3$s} & \multirow{2}{*}{$264.4$s} & $31.2$s ($14.6$s) \\
        \cline{9-9} 
        & & & & & & & & \textbf{$\bm{0.66}$s} (\textbf{$\bm{0.62}$s}) \\
        \hline
        Cart-Pole & $7.5$s & $147.1$ms & $588.2$ms & \textbf{$\bm{29.1}$ms} & \textbf{$\bm{112.0}$s} & $1471$s & $3671$s & $183.0$s ($173.1$s) \\
        \hline 
        Car Back-in & $778.1$s & $612.3$ms & $1.8$s & $\bm{44.8}$\textbf{ms} & $>5$h & $6123$s & $>5$h & \textbf{$\bm{431.5}$s} (\textbf{$\bm{536.8}$s})  \\
        \hline 
        Vehicle Landing & $1387$s & $1.0$s & $2.4$s & $\bm{118.3}$\textbf{ms} & $>5$h & $2.9$h & $>5$h &  \textbf{$\bm{919.2}$s} (\textbf{$\bm{1165}$s}) \\
        \hline 
        Flying Robot & - & $1.7$s & $6.2$s & $\bm{169.7}$\textbf{ms} & - & $>5$h & $>5$h & \textbf{$\bm{1648}$s} (\textbf{$\bm{2027}$s}) \\
        \hline 
    \end{tabular}
    }

    \caption{Per-interation costs and total time costs for different solvers across five experiments. For \cuadmm, we report the means (medians) of total time costs. The pendulum case lists total time costs with (upper) and without (lower) warm starts. For the flying robot case, \MOSEK runs out of 1TB memory.}
\end{table}
